CO-NNECT: A Framework for Revealing Commonsense Knowledge Paths as Explicitations of Implicit Knowledge in Texts

In this work we leverage commonsense knowledge in form of knowledge paths to establish connections between sentences, as a form of explicitation of implicit knowledge. Such connections can be direct (singlehop paths) or require intermediate concepts (multihop paths). To construct such paths we combine two model types in a joint framework we call Co-nnect: a relation classifier that predicts direct connections between concepts; and a target prediction model that generates target or intermediate concepts given a source concept and a relation, which we use to construct multihop paths. Unlike prior work that relies exclusively on static knowledge sources, we leverage language models finetuned on knowledge stored in ConceptNet, to dynamically generate knowledge paths, as explanations of implicit knowledge that connects sentences in texts. As a central contribution we design manual and automatic evaluation settings for assessing the quality of the generated paths. We conduct evaluations on two argumentative datasets and show that a combination of the two model types generates meaningful, high-quality knowledge paths between sentences that reveal implicit knowledge conveyed in text.

==> add-red.tex <==
@inproceedings{callison-burch-etal-2006-evaluating,
    title = "Re-evaluating the Role of {B}leu in Machine Translation Research",
    author = "Callison-Burch, Chris  and
      Osborne, Miles  and
      Koehn, Philipp",
    booktitle = "11th Conference of the {E}uropean Chapter of the Association for Computational Linguistics",
    month = apr,
    year = "2006",
    address = "Trento, Italy",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/E06-1032",
}

@inproceedings{paul-frank-2020-social,
    title = "Social Commonsense Reasoning with Multi-Head Knowledge Attention",
    author = "Paul, Debjit  and
      Frank, Anette",
    booktitle = "Findings of EMNLP",
    year = "2020",
    pages = "2969--2980",
}

@inproceedings{chang-etal-2020-incorporating,
    title = "Incorporating Commonsense Knowledge Graph in Pretrained Models for Social Commonsense Tasks",
    author = "Chang, Ting-Yun  and
      Liu, Yang  and
      Gopalakrishnan, Karthik  and
      Hedayatnia, Behnam  and
      Zhou, Pei  and
      Hakkani-Tur, Dilek",
    booktitle = "DeeLIO",
    year = "2020",
    pages = "74--79",
}


@inproceedings{habernal-etal-2018-argument,
    title = "The Argument Reasoning Comprehension Task",
    author = "Habernal, Ivan  and
      Wachsmuth, Henning  and
      Gurevych, Iryna  and
      Stein, Benno",
    booktitle = "NAACL",
    year = "2018",
    %address = "New Orleans, Louisiana",
    %url = "https://www.aclweb.org/anthology/N18-1175",
    %doi = "10.18653/v1/N18-1175",
    pages = "1930--1940"
}

  
@inproceedings{vylomova-etal-2016-take,
    title = "Take and Took, Gaggle and Goose, Book and Read: Evaluating the Utility of Vector Differences for Lexical Relation Learning",
    author = "Vylomova, Ekaterina  and
      Rimell, Laura  and
      Cohn, Trevor  and
      Baldwin, Timothy",
    booktitle = "the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = aug,
    year = "2016",
    address = "Berlin, Germany",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P16-1158",
    doi = "10.18653/v1/P16-1158",
    pages = "1671--1682",
}

@inproceedings{trisedya-etal-2019-neural,
    title = "Neural Relation Extraction for Knowledge Base Enrichment",
    author = "Trisedya, Bayu Distiawan  and
      Weikum, Gerhard  and
      Qi, Jianzhong  and
      Zhang, Rui",
    booktitle = "the 57th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2019",
    address = "Florence, Italy",
    url = "https://www.aclweb.org/anthology/P19-1023",
    doi = "10.18653/v1/P19-1023",
    pages = "229--240"
}




@inproceedings{guo-etal-2019-attention,
    title = "Attention Guided Graph Convolutional Networks for Relation Extraction",
    author = "Guo, Zhijiang  and
      Zhang, Yan  and
      Lu, Wei",
    booktitle = "the 57th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2019",
    address = "Florence, Italy",
    url = "https://www.aclweb.org/anthology/P19-1024",
    doi = "10.18653/v1/P19-1024",
    pages = "241--251",
}
